SchedGuard: Protecting against Schedule Leaks Using Linux Containers

Real-time systems have recently been shown to be vulnerable to timing inference attacks, mainly due to their predictable behavioral patterns. Existing solutions such as schedule randomization lack the ability to protect against such attacks, often limited by the system's real-time nature. This paper presents SchedGuard: a temporal protection framework for Linux-based hard real-time systems that protects against posterior scheduler side-channel attacks by preventing untrusted tasks from executing during specific time segments. SchedGuard is integrated into the Linux kernel using cgroups, making it amenable to use with container frameworks. We demonstrate the effectiveness of our system using a realistic radio-controlled rover platform and synthetically generated workloads. Not only is SchedGuard able to protect against the attacks mentioned above, but it also ensures that the real-time tasks/containers meet their temporal requirements.

==> bck_2_model.tex <==
\section{Scheduler design}
\label{sec:design}


Containers are implemented with primitives of the Linux kernel, namespaces and cgroups, to provide OS level virtualization. 
Namespaces partition system resources by restricting what processes can see such that the resources appear to be dedicated to the processes. 
Cgroups control and limit the amount of system resources that are allocated to a group of processes, such as CPU, memory size, disk I/O, etc..
In terms of scheduling, container can be viewed as equivalent to cgroups.  (\textcolor{red}{might need to change wording})
For a group of real-time processes, it can also be used to control how much CPU time at maximum can be used for real-time execution.
Each group is associated with a real-time runtime and period, which limits the maximum runtime processes belonging to that group is allowed to run for each period. 
This interface can be used to implement a hierarchical scheduling framework. 
The Predictable real-time scheduler for container extends the existing cgroups property to provide more strict temporal isolation for processes. 

\textcolor{red}{Add high level figure}

\todo[inline]{Naming suggestion: Maybe assign specific names to first/second level. Like container (first) and task(second) scheduler}

The scheduler adopts a two level scheduling framework.
On the first level, the scheduler assigns fixed \todo{What does fixed mean? Ordering is not fixed, only max time is. Also comma not required}%
, non-preemptable time slot for different containers. 
The second level scheduler is fixed priority based and chooses the highest priority process to run.\todo{reword: The second level scheduler, i.e. scheduling tasks belonging to a container, is based on static priorities.}

\subsection{First level scheduler}

The first level scheduler assigns real-time runtime and period for different containers, using the cgroups interface. 
However, unlike default Linux scheduling behavior, this runtime has to be continuous and does not allow preemption from other containers, no matter how high the priority of the competing process is. 
This guarantees the container and its processes can have this runtime by themselves without interruption from outside tasks. 
The container will be descheduled only if: 1. The runtime has been used up for that period. 2. There are no running processes or ready tasks waiting for execution in that container during that period. 
This descheduling mechanism works similar to the Timed Token Ring scheduler with maximum holding time. 
However, the decision to switch container or not is completely determined by the kernel scheduler, not user tasks. 
This makes the system more robust that even if one task is compromised and runs long, it can't occupy the CPU more than the assigned time slot. 

Each container's priority is determined by the highest priority task inside it.
When choosing the next container to run, the scheduler simply picks the highest task available and thus selecting the corresponding container to run.
This also has the advantage that once a faulty process got boosted somehow, the execution order between containers will change, making it easy for fault detection.


The first level scheduler is implemented directly on the Linux real-time scheduler code for SCHED\_FIFO and SCHED\_RR.
In order to schedule real-time processes in cgroups, CONFIG\_RT\_GROUP\_SCHED is enabled when compiling the kernel.
A new scheduling class SCHED\_IMA is added to differentiate from existing scheduling classes. 
To implement the new scheduling logics, two major concerns should be addressed:
\begin{itemize}
  \item The container cannot be preempted by other tasks.
  \item When one task finishes, the scheduler should first look at tasks in the same container.
\end{itemize}
For the first point, in the scheduler function check\_preempt\_curr\_rt() four checks are added to implement the strict non-preempting rule in the IMA style for the SCHED\_IMA(\textcolor{red}{need to make sure this is correct}).

\begin{itemize}
  \item If the currently running task belongs to the SCHED\_IMA class.
  \item If the current real-time runqueue's runtime has been exhausted. 
  \item If the new real-time task belongs to the SCHED\_IMA class.
  \item If the new task and the current task belongs to the same rt\_runqueue, which means they are from the same cgroup.
\end{itemize}

Only after all fours checks have been passed is it allowed for preemption to happen.
For the second point, in the function \_pick\_next\_task\_rt() the scheduler will check if the current task belongs to SCHED\_IMA class. 
If the answer is yes, the scheduler will look for available tasks in that cgroup's runqueue first, ignoring system wide process priority. 
If the answer is no or there are no tasks can execute in that container, it will fall back to original task picking process.


\subsection{Second level scheduler}


The second level scheduler schedules container tasks with fixed priority during the assigned runtime. 
Currently, only original Linux real-time schedulers SCHED\_FIFO and SCHED\_RR are supported.
Since the SCHED\_DEADLINE scheduler has its own scheduling class (deadline class), it is not supported yet. 


Here's an example showing how the scheduler differs from SCHED\_FIFO scheduler in Linux.
Consider a task set \( \Gamma =\left \{ {\tau _{1}, \tau _{2}, \tau _{3}} \right \} \), with \(\tau _{1} \) and \(\tau _{3} \) are periodic tasks and \( C_{1}=C_{3}=10ms, P_{1}=P_{3}=100ms \), while \(\tau_{2}\) runs all the time and \(C_{2}=\infty，P_{2}=\infty\).
Also assume that the task set has descending priority, such that \(\tau _{1}\) has the highest priority and \(\tau _{3}\) has the lowest one. 
\(\tau _{1} \) and \(\tau _{3} \) are put inside one container and has a runtime larger than 20ms per 100ms period. \(\tau _{2} \) lives in a separate container by itself.
With the Linux default SCHED\_FIFO scheduler, \(\tau _{3} \) would never get a chance to execute as \(\tau _{2} \) has higher priority and would take all the available CPU time. 
However, using the new predictable scheduler \(\tau _{3} \) runs right after \(\tau _{1} \) since they belong to the same container. 
Even though \(\tau _{2} \) has high priority, it is not allowed to preempt the execution of the running container. 

% Here is an example of the execution order of three example tasks:
% ff\_30\_infi has priority 30 and runs continuously on the host system. 
% alarm\_40 and alarm\_20 are two periodic tasks running inside a container. 
% All three processes run on core 0.
% Using the system default FIFO scheduler, the alarm\_20 does not have a chance to run because it has the lowest priority among the three processes (it's not shown in the picture because it doesn't run). 
% However, using the new scheduler it runs right after alarm\_40 since they belong to the same container. 
% Even though ff\_30\_infi has high priority, it is not allowed to preempt the execution of the running container. 



% The scheduler adopted a two level scheduling framework: on the first level, the scheduler assigns time slices for different containers. 
% Each container will be assigned some dedicated time slots in each period.
% The second level scheduler which is inside the container will schedule container tasks for those time slots. 




% \subsubsection{new scheduler}

% The new scheduler has advantages of both the Timed Token Ring scheduler and the TDMA scheduler. 
% The scheduler chooses container to run based on the highest priority of the ready tasks of a container.
% In the assigned time slot, only tasks belonging to that container are allowed to execute.
% Tasks from other containers are not allowed to preempt the execution of current container, regardless of their system wide priorities. 
% However, if there are no tasks waiting for execution inside the running container, the system scheduler will yield the CPU to other containers. 
% Unlike Timed Token Ring scheduler, the decision to switch container or not is fully determined by the system scheduler, not user task. 
% This has the advantage that even if one task is compromised and runs long, it can't occupy the CPU more than the assigned time slot. 


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/old_order.png}\vspace{-1em}
  \caption{Order of execution under original FIFO scheduler}
  \label{fig:call}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/new_order.png}\vspace{-1em}
  \caption{Order of execution under new scheduler}
  \label{fig:call}
\end{figure}

\textcolor{red}{needs better graphics}



At this stage the scheduler is designed only for single core processes. 
Due to the resource contention problem that would occur when scheduling real-time processes on multi-core platform \textcolor{red}{cite SCE paper}, the scheduler does not support multi-core for the time being. 



% \subsubsection{Timed Token Ring scheduler}

% The Timed Token Ring scheduler takes the idea from distributed network scheduling. 
% Each container is given time slots based on a predetermined time table. 
% The length of time slots should allow the tasks running inside the containers to finish before deadline.
% Containers can choose to yield if tasks finish early and there is still time left, but preemption from another container is not allowed. 
% (This is basically a more flexible RR scheduler on the Linux system.)
% However, in the case a task needs to wait for input data, it cannot yield until that task has finished. 

% The Timed Token Ring scheduler is implemented based on the Round Robin scheduler in the Linux system. 
% Instead of a fixed 10ms time slice, the scheduler provides a configurable time slice, ranging from 1 to 100ms. 


% \subsubsection{TDMA scheduler}

% The TDMA scheduler has tighter requirement on the scheduling behavior. No preemption is allowed and container cannot yield even if there are still time left for that time slot.




==> old file/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%structure 1:
%With numbers, we can say VM is very slow. 

%Structure 2:
%we only focus on container part, with this IMA framework. 

One of the major design goal of the IMA architecture is to allow hardware resources such as processor and memory subsystem to be shared by the software running in different criticality domains. 
While achieving such goal, requirements such as partitioning has to be enforced. Partitioning in IMA suggests that an applications running in one criticality domain should not affect the timing/behavior of an application in another criticality domain. 

To achieve aforementioned partitioning goal suggested by IMA design. In this work, we propose the use of Linux Containers. Container is a lightweight virtualisation technology that offers isolation to application without the overhead of Virtual Machine (VM). Linux inherently supports containers and allows us to schedule them using different scheduling mechanisms such as CFS, FIFO and RR. While these scheduling mechanisms are great for average case performance. They do not assure any real-time guarantees.    

% \todo[inline]{RT:add other related works here and mention differences briefly}

To support real-time scheduling framework for Linux containers. In this work, we propose RT-Containers. RT-Containers ensure strong timing isolation between different containers such that no container can hold the resources (CPU and memory) forever. RT-Container provides such isolation by proposing two-level of scheduling. The first-level of scheduling (between containers) allows us to schedule the containers using TDMA. Whereas, the second-level of scheduling allows us to run multiple processes inside a container. To summarize, the major contribution of this work are as follows:    

%, there is yet a real-time scheduler for container that is compatible with IMA standard. 
%The proposed two level scheduling framework can make sure no container can hold the CPU forever. 
%Once its time slice is used up the container is scheduled out as a whole, saving other containers from starvation. (safety)
%Safety is very important and separation of concerns is the basis of safety critical automotive and avionics systems. 

\begin{itemize}
  \item We propose a two level real-time scheduling framework for Linux containers (called RT-Containers). The first level can be configured as either TDMA or Timed token ring, depending on the needs. The second level scheduler is Rate Monotonic.
  \item The first-level of scheduler in the RT-Container adheres to paritioning goal of IMA design. 
  %\item We provide real-time schedulability analysis for our framework. 
  %\item We present initial experiment results to show the feasibility of our proposed approach.
  \item We evaluate our proposed framework and compare it with that of traditional container scheduling approaches offerred by Linux.  
\end{itemize}


\section{Background}
\label{sec:background}



\subsection{IMA}





\subsection{Containers}

Real time applications have different critically requirements and relies on different software components and keeping them in different environment is a crucial problem.
Virtual machine (VM) have been used extensively in isolating different applications in separate environments. 
Each VM virtualize its own hardware stack and runs its own operating system.
A hypervisor normally exists to organize different VMs, allocating host system resources according to their needs. 
Though successful in providing a good isolation, VM still has some drawbacks. 
They consume large amount of system resources due to the need to virtualize both hardware and software components. 
For certain applications this is an overkill. 
Because of the level of virtulization, VM's performance is worse than the host system process. 
Even with para-virtualizaiton it is still not on the same level. 
VM is also known to start quite slow, usually measured in minutes. 


Container is another way of virtualizing the underlying computer.
Instead of virtualizing the entire OS and hardware stack, it shares the host OS kernel and only emulates the operating system 
\cite{merkel2014docker,preeth2015evaluation}. 
On Linux, it uses Linux kernel features, like Control Groups (cgroups), Namespace to provide spacial isolation and system resource allocation on the host OS. 
Though sharing the host kernel brings some security concerns, it makes container much lightweight compared with VM.
Due to the reduced level of separation, container has less execution overhead and less memory usage.
They are normally megabytes in size and can start in seconds. 
This also means with the same hardware resources one can run more containers than VMs, hosting more applications and producing more throughput. 


After many years of development, there are now many tools developed that make it much easier to develop, ship and deploy applications with containers. (examples and references needed)
Nowadays, container is mainly used on cloud to host network microservices, such as Google Cloud and Amazon cloud. (needs citations and expand more) 
Due to the reduced memory footprint, containers allow the same server to host more applications running in their own isolated environment simultaneously. 
Breaking large applications into microservices and hosting them in containers also makes it easier to upgrade existing applications. 
Many consider container to be not as safe as VMs (needs citatation) so their usage is scarce in areas where security is a important concern. 
However, container has their own advantage in terms of security compared with VMs. 
Some of the most common seen vulnerabilities in VM come from outdated software packages. 
With a monolithic structured application, it often runs for a long period of time in VM before it can be patched by application maintainers. 
For containers, it's more convenient to release new version of software that has updated packages and has been patched for known vulnerabilities. 
Due to a modularized structure, an application is split to run in several containers which reduces the outcome of any exploit. 
Individual components that run in containers can also be restarted in a short time once any abnormal behavior is detected. 
As a result, container can still be used as a virtuliazation to host non-network oriented services, such as real-time applications. (emphasize security at here?)


% \subsection{Real-Time Applications}







% Container is a popular open-source technology that provides lightweight software isolation \cite{merkel2014docker,preeth2015evaluation}. 
% In its core, it is an abstraction of several features in Linux kernel. 
% Control Groups (cgroups) provides resource allocation, such as CPU and memory. 
% Namespace isolates processes so each has a different view of the system. 
% Other modules like SELinux \cite{smalley2001implementing}, AppArmor \cite{apparmor}, Seccomp \cite{seccomp} provide container security capabilities \cite{bui2015analysis}. 
% Instead of virtualizing an entire operating system, containers provide only the bare minimum requirements for the application to run and multiple containers share the host operating system kernel. On the host system, each container is just a process running the application and necessary dependencies. 
% System isolation using containers leads to less execution overhead, less memory usage, and reduced footprint. 


% Compared with virtual machines, containers have several advantages \cite{dockerintro}:
% \begin{itemize}
%     \item Lightweight: Containers share the host's kernel while the virtual machine needs a hypervisor to talk to the kernel and the underlying hardware. 
%     \item Efficiency: The average size of a container is around tens of MB while a VM easily exceeds GB. More containers can run on the same machine at the same time than VMs could which means the same computing resource may generate more results using containers. 
%     \item Portability: Containers have developed over the years and evolved from a Linux only application to be able to run virtually anywhere: on Mac and Windows operating system; on bare metal and public cloud. It greatly reduces the effort for development and time for deployment. 
% \end{itemize}


==> old file/2_model.tex <==
\section{Scheduler design and implementation}
\label{sec:design}

% \todo[inline]{Reocmmendation: If short paper let's merge design and implementaion, which seems to be the case currently too. If long paper, they can be separated so they occupy more space.}

Linux kernel provides two primitives that form the backbone of virtualization in container framework, namespaces and cgroups.
Namespaces virtualize system resources by first, restricting visibility of resources to process and second, by making the resources seem fully dedicated to processes.
Cgroups control and limit the amount of system resources that are allocated to a group of processes, such as CPU, memory size, disk I/O, etc..
In standard container implementations processes belonging to containers are scheduled as independent processes but in this work we create another level so that processes belonging to a container can be scheduled as a combined entity. This is achieved by leveraging cgroups.
Thus groups of real-time processes can be grouped together in containers and the group itself scheduled with predictable resource allocations and uppoer bounds.
Each group has an associated execution time and period, which limits the maximum runtime processes belonging to that group is allowed to run over a duration of time.
This interface is thus used here to implement a hierarchical scheduling framework. 
The predictable real-time scheduler for container extends the existing cgroups property to provide strict temporal isolation for processes. 

% \todo[inline]{Add high level figure}

The scheduling logic proposed and implemented in this work adopts a two level scheduling approach.
On the first level called \textit{Container scheduler}, is a Timed Token Ring scheduler that under specific configurations can be made equivalent to a TDMA scheduler.
The second level called \textit{Task scheduler} is a fixed priority scheduler.

\subsection{Container scheduler}

The processor time is broken up into equal sized periods, 100 ms default. The container scheduler allows the system administrator to assign each container a percentage of this global period. Each container can also be assigned a relative priority. If container level priorities are not assigned, they inherit the priority of their highest priority ready task. At the start of each period the container with highest assigned or inherited priority is chosen to run. Once selected the container is not preempted till it either utilizes its assigned portion of the period or has no tasks remaining that can be run. This behavior is implemented using the cgroups interface.

Unlike default Linux scheduling behavior, the proposed scheduler does not allow preemption from other containers, independent of the priority of the competing processes.
This guarantees the container and its processes, once chosen by scheduler, will have no interruptions from outside tasks, during their assigned runtime.
The decision to preempt a container when it has used its allocated time is completely determined and enforced by the kernel scheduler.
This makes the system robust and even if a task is compromised and runs long, the containing container can not exceed the assigned time slot.

With no additional configuration, container selection withing a period is based on the priority of the highest priority task that is ready to run within each container. Once a container is chosen, it fully executes all ready tasks or till it completely uses its time slot. After this one of the other containers is chosen based on same logic. Within a period a container is only chosen once.
This makes the default scheduler behave like a Timed Token Ring with restricted max token hold time. 



\subsection{Task scheduler}
The Task scheduler selects tasks from the currently running container based on fixed priority. 
% \todo[inline]{@Jiyang - are other options possible? Like FIFO/RR/DEADLINE? Is that what the next two sentences say? Yes.}
Currently, the supported scheduling policy are  Linux real-time policy SCHED\_FIFO and SCHED\_RR.
The SCHED\_DEADLINE scheduler has a seperate scheduling class (deadline class) with the two real-time class which makes it not supported yet. 

\subsection{Implementation}
The container scheduler is implemented as a new Linux real-time scheduler SCHED\_IMA.
Compared to existing Linux real-time scheduler it has three distinction features:
\begin{itemize}
  \item A running container cannot be preempted by tasks from other containers.
  \item Upon task completion, the scheduler should first exhaust tasks from the same container.
  \item Forced preemption of tasks when the container time slot is used up.
\end{itemize}

% \todo[inline]{Do we need the below level of detail in implementation? Also we should have open source patch at least. RTCSA is single blind so link to such a patch should be included in the submitted paper.}

These are achieved by modifying the way Linux check real-time task preemption and how new real-time tasks are picked from the available runqueue. 
For strict non-preempting rule in the IMA style, four rules has to be met in order for task preemption to take place:

\begin{itemize}
  \item The currently running task belongs to the SCHED\_IMA class.
  \item The current real-time runqueue's runtime has not been exhausted.
  \item The new real-time task belongs to the SCHED\_IMA class.
  \item The new task and the current task belongs to the same rt\_runqueue.
\end{itemize}

Besides these, the only way preemption can happen is when the rt\_runqueue's runtime has been exhausted. 

When task finishes execution, the scheduler will first look for tasks from the current task's rt\_runqueue.
This effectively ignores system wide process priority, but only focus on priority assigned inside individual containers. 
Only when the rt\_runqueue is throttled due to no runtime left or there are no tasks available in that container, will the scheduler fall backs to select task based on system wide priority. 

\subsection{Comparisons}

Here's an example showing how the scheduler differs from SCHED\_FIFO scheduler in Linux.
Consider a task set \( \Gamma =\left \{ {\tau _{1}, \tau _{2}, \tau _{3}} \right \} \), with \(\tau _{1} \) and \(\tau _{3} \) are periodic tasks and \( C_{1}=C_{3}=10ms, P_{1}=P_{3}=100ms \), while \(\tau_{2}\) runs all the time and \(C_{2}=\infty，P_{2}=\infty\).
Also assume that the task set has descending priority, such that \(\tau _{1}\) has the highest priority and \(\tau _{3}\) has the lowest one. 
\(\tau _{1} \) and \(\tau _{3} \) are put inside one container and has a runtime larger than 20ms per 100ms period. \(\tau _{2} \) lives in a separate container by itself.
With the Linux default SCHED\_FIFO scheduler, \(\tau _{3} \) would never get a chance to execute as \(\tau _{2} \) has higher priority and would take all the available CPU time. 
However, using the new predictable scheduler \(\tau _{3} \) runs right after \(\tau _{1} \) since they belong to the same container. 
Even though \(\tau _{2} \) has high priority, it is not allowed to preempt the execution of the running container. 

% Here is an example of the execution order of three example tasks:
% ff\_30\_infi has priority 30 and runs continuously on the host system. 
% alarm\_40 and alarm\_20 are two periodic tasks running inside a container. 
% All three processes run on core 0.
% Using the system default FIFO scheduler, the alarm\_20 does not have a chance to run because it has the lowest priority among the three processes (it's not shown in the picture because it doesn't run). 
% However, using the new scheduler it runs right after alarm\_40 since they belong to the same container. 
% Even though ff\_30\_infi has high priority, it is not allowed to preempt the execution of the running container. 



% The scheduler adopted a two level scheduling framework: on the first level, the scheduler assigns time slices for different containers. 
% Each container will be assigned some dedicated time slots in each period.
% The second level scheduler which is inside the container will schedule container tasks for those time slots. 




% \subsubsection{new scheduler}

% The new scheduler has advantages of both the Timed Token Ring scheduler and the TDMA scheduler. 
% The scheduler chooses container to run based on the highest priority of the ready tasks of a container.
% In the assigned time slot, only tasks belonging to that container are allowed to execute.
% Tasks from other containers are not allowed to preempt the execution of current container, regardless of their system wide priorities. 
% However, if there are no tasks waiting for execution inside the running container, the system scheduler will yield the CPU to other containers. 
% Unlike Timed Token Ring scheduler, the decision to switch container or not is fully determined by the system scheduler, not user task. 
% This has the advantage that even if one task is compromised and runs long, it can't occupy the CPU more than the assigned time slot. 


\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/old_order.png}\vspace{-1em}
  \caption{Order of execution under original FIFO scheduler}
  \label{fig:old_order}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/new_order.png}\vspace{-1em}
  \caption{Order of execution under new scheduler}
  \label{fig:new_order}
\end{figure*}

% \todo[inline]{needs better graphics}


\subsection{Limitations}
The current IMA scheduler is designed for  single core scheduling only. 
Resource contention~\cite{sce} among real-time processes on multi-core platforms cannot be solved with scheduler alone. Hence IMA standards cannot be met on multi-core platforms by scheduler design alone. A combination of Single Core Equivalence and RT Containers can be used though and will be explored further in future work.



% \subsubsection{Timed Token Ring scheduler}

% The Timed Token Ring scheduler takes the idea from distributed network scheduling. 
% Each container is given time slots based on a predetermined time table. 
% The length of time slots should allow the tasks running inside the containers to finish before deadline.
% Containers can choose to yield if tasks finish early and there is still time left, but preemption from another container is not allowed. 
% (This is basically a more flexible RR scheduler on the Linux system.)
% However, in the case a task needs to wait for input data, it cannot yield until that task has finished. 

% The Timed Token Ring scheduler is implemented based on the Round Robin scheduler in the Linux system. 
% Instead of a fixed 10ms time slice, the scheduler provides a configurable time slice, ranging from 1 to 100ms. 


% \subsubsection{TDMA scheduler}

% The TDMA scheduler has tighter requirement on the scheduling behavior. No preemption is allowed and container cannot yield even if there are still time left for that time slot.




==> old file/33_model.tex <==
\newpage
% To check if existing lower priority tasks can cover the window, the following conditions have to be matched:

% \[\sum^{i} \left \lceil \frac{P_{g,l}}{P_{g,i}} \right \rceil \cdot C_{g,i} \geq \left \lceil \frac{P_{g,l}}{P_p} \right \rceil w_e\]

% (need to add additional check to make sure each instance is covered, not just the total sum)



\subsection{Attacker/untrusted tasks are of a priority higher than the victim}

This considers the case where untrusted tasks can also be higher priority than the victim task.

For higher priority untrusted tasks, the attack effective window introduces additional blocking which is 
\(w_e\). 


\subsection{Check schedulability of higher priority task}
When the guard tasks are lower priority tasks or idle task, schedulability of all higher priority task will be affected. 

\[r_{i}^{k+1} = C_i + w_e + \sum_{j=1}^{i-1} \left \lceil \frac{r_{i}^{k}}{P_j} \right \rceil \cdot C_j, r_{i}^{0} = \sum_{j=1}^{i} \cdot C_j + w_e\]

\tk{Can we relax the assumption that the attacker has the lowest priority? Task should not be blocked if we know that it cannot do any harm to the victim task.}

\tk{Since the task effective window is non-preemptive, the above model complies with the Fixed Preemption Points (also known as Cooperative Scheduing)~\cite{Bril2007,Buttazzo2013,Burns1995}.}

If any higher priority task fails the response time analysis, it means the current task set cannot be protected using the proposed defense mechanism. 
However, in later section we'll discuss a way to improve the response time of a trusted high priority task. 


\subsection{Use lower priority tasks to block attack effective window}

Here we discuss the case where all guard tasks \(\tau_g\) are composed of lower priority tasks of the victim task \(\tau_v\).
In this case, schedulable lower priority tasks will remain schedulable. 
To determine the guard tasks set, we need to make sure the attack effective window can be covered by the task sets. 
That is,

\[\sum^{i} \left \lceil \frac{P_{g,l}}{P_{g,i}} \right \rceil \cdot C_{g,i} \geq \left \lceil \frac{P_{g,l}}{P_p} \right \rceil w_e\]

where \(\tau_{g,l}\) is the lowest priority task among all guard tasks \(\tau_{g,i}\) and \(P_{g,l}\) is its period. 
\(\tau_{g,i}\) refers to a guard task.
The left hand side of the equation is the sum of execution time of all guard tasks in \(P_{g,l}\).
The right hand side is the sum of all attack effective window in \(P_{g,l}\).
% Considering the performance impact of running processes inside container\cite{morabito2017virtualization}, use \(s\) to denote container slow down factor. 
If the above condition does not hold, one should keep adding lower priority trusted tasks into the guard task set, or use idle task to fill the unfulfilled time. 
The case where idle task is used will be discussed in later section. 

\tk{Example. 
Let $\tau_p=(1,5)$, $\tau_g=(3,7)$ and $w_e=1$. Since task $\tau_g$ is the only guard task $P_{g,l}=P_{g}$. The above relation holds, $1 \cdot 3 \geq 2 \cdot 1$, but only the first window is covered, the second and the third are not.}
\begin{figure}[hbt]
\begin{center}
\begin{RTGrid}[width=.45\textwidth,nosymbols=1,nogrid=0,nonumbers=0,numbersize=\footnotesize]{2}{15}
\RTBox{1}{2}
\RTBox{6}{7}
\RTBox{11}{12}

\RowLabel{1}{$\tau_p$}
\TaskArrival{1}{0}
\TaskArrival{1}{5}
\TaskArrival{1}{10}
\TaskExecution{1}{0}{1}
\TaskExecution[color=blue!50,execlabel=$w_e$]{1}{1}{2}
\TaskExecution{1}{5}{6}
\TaskExecution[color=blue!50,execlabel=$w_e$]{1}{6}{7}
\TaskExecution{1}{10}{11}
\TaskExecution[color=blue!50,execlabel=$w_e$]{1}{11}{12}

\RowLabel{2}{$\tau_g$}
\TaskArrival{2}{0}
\TaskArrival{2}{7}
\TaskArrival{2}{14}
\TaskExecution{2}{1}{4}
\TaskExecution{2}{7}{10}
\end{RTGrid}
\end{center}
\caption{Attack window overlapping with low priority tasks.}
    \label{fig:example_1}
\end{figure}

\tk{If victim task executes less that its worst-case execution time and the guard task is released after the victim task, the victim task  might be exposed to the attacker. We may need to assume that the task execution does not vary (i.e. task always occupies the processor for the worst-case execution time).}

\tk{In~\cite{nasri2019pitfalls} Lemma 4 gives a condition when attacker has higher priority. By assigning the higher priority to the attacker, the attack is less likely to be successful. }
\jy{That lemma also assumes that the victim task and the attacker task are harmonic.}

For a guard tasks \(\tau_{g,i}\), if all its execution time is used to occupy the attack effective window, the response time is determined by the number of window it gets executed, denoted by \(k\).
\(\tau_{g,j}\in hp(\tau_{g,i})\) refers to all higher priority guard tasks than the task \(\tau_{g,i}\).
\(\tau_{g,i}\) can only execute after higher priority guard tasks have finished execution.

\[k = \left \lceil \frac{\sum_{\tau_{g,j}\in hp(\tau_{g,i})}^{}C_{g,j}+C_{g,i}}{w_{e}} \right \rceil\]
% \[k = \left \lceil s \cdot \frac{\sum_{\tau_{g,j}\in hp(\tau_{g,i})}^{}C_{g,j}+C_{g,i}}{w_{e}} \right \rceil\]
Suppose we already have the response time of the victim task \(\tau_v\) as \(r_p\).
The response time of guard task is

\[r_g = (k-1) \cdot P_p + r_p + (\sum_{\tau_{g,j}\in hp(\tau_{g,i})}^{}C_{g,j}+C_{g,i}) - (k-1) \cdot w_e  \]
% \[r_g = (k-1) \cdot P_p + r_p + s \cdot (\sum_{\tau_{g,j}\in hp(\tau_{g,i})}^{}C_{g,j}+C_{g,i}) - (k-1) \cdot w_e  \]

If execution time of \(\tau_{g,i}\) is partially used to cover the attack effective window, which also means it's the lower priority task in the guard task set, we can model it as a task with the same priority and period but with less execution time. 
The new execution time will be 

\[C_i = \sum_{\tau_{g,j} \in hp(\tau_{g,i})} C_{g,j} + C_{g,i} - k \cdot w_e \]
% \[C_i = s \cdot (\sum_{\tau_{g,j} \in hp(\tau_{g,i})} C_{g,j} + C_{g,i}) - k \cdot w_e \]

which is the residue execution time after executing in attack effective window.
With this new \(C_i\), one can use the standard response time analysis. 

\subsection{Use idle task to block attack effective window}

\ab{this is the easiest case to reason about, so put it first. Also the guard task terminology is making this over complicated. idle task is the guard task in this case. So Cidle = window and period of idle task is same as period of victim task. Right? Am I missing something here?}
\jy{This is the case where a single idle task is used as guard task or a mix of existing task and idle task is used.}

 
Since every task in the system is periodic, the need for idle task to fill the attack effective window also comes in a periodic way. 
Model the idle task \(\tau_{idle}\) as \((C_{idle}, P_{idle})\) where \(C_{idle}\) is 

\[C_{idle} = \left \lceil \frac{P_{g,l}}{P_p} \right \rceil w_e - \sum_{\tau_{g,i}\in hp(\tau_p)}^{i} \left \lceil \frac{P_{g,l}}{P_{g,i}} \right \rceil C_{g,i} \]
% \[C_{idle} = \left \lceil \frac{P_{g,l}}{P_p} \right \rceil w_e - \sum_{\tau_{g,i}\in hp(\tau_p)}^{i} \left \lceil \frac{P_{g,l}}{P_{g,i}} \right \rceil s\cdot C_{g,i} \]

and \(P_{idle}\) is 

\[P_{idle} = \left \lceil \frac{P_{g,l}}{P_p} \right \rceil P_p\]

If idle task is the only guard task, \(P_{idle}\) equals to \(P_{p}\).
With the introduction of a idle task, schedulability of lower priority task will also be affected.
During response time analysis, the priority of the idle task can be set as just below the lowest guard task.
All task with equal or lower priority than this idle task should consider it during response time analysis. 


\subsection{Use higher priority task to block attack effective window}

If there is a higher priority trusted task in the system that is missing the deadlines after introducing the non-preemptive attack effective window, one can add it to the guard task so it can execute during the attack effective window. 
Since the original task set is schedulable, giving the task permission to execute during the attack effective window will reduce its worst case response time. 
The task can be made schedulable as long as it can execute for \(w_{e,h}\) in the attack effective window, and \(w_{e,h}\) is 

\[ w_{e,h} = r_{i}^{k} - P_i \]
% \[w_{e,h} = (r_{i}^{k} - P_i) \cdot s\]

\(r_{i}^{k}\) is the smallest response time of this task that is greater than \(P_i\) calculated using standard response time analysis after considering the blocking attack effective window.
\(w_{e,h}\) is guaranteed to be smaller than \(w_{e}\).
The remaining time in the attack effective window can be occupied with lower priority task or idle task as have explained above. 

==> old file/3_implementation.tex <==

\section{Implementation}
\label{sec:implementation}


Notes:

Add configurable handling for first level of scheduler so that the container level scheduling is one of
\begin{enumerate}
    \item Inherited from highest runnable task from the container : this has the best response time for highest priority tasks in the system, but container execution order is not predictable. A faulty taask in a container can keep changing the order of execution of containers.
    \item Administrator configurable relative priorities of containers which then is used to order containers withing time slices. Among equal priority container the order can be based on the above approach. Benefit : container execution order is maintained independent of faults. Still flexible.
\end{enumerate}
 If all containers have assigned and unique priorities, level 1 is TDMA. If none of the containers have assigned priorities, level 1 becomes timed token ring.



==> old file/4_eval.tex <==
\section{Evaluation}

\subsection{Fault tolerance}
This experiment aims to show that if a task goes wrong, only the associate container is affected. 
The other container's runtime, potentially execution order, will not be affected. 
\begin{enumerate}
    \item Create a task set with 6 tasks. Capture their completion time and any deadline misses. Ensure that there are no deadlines missed in this scenario. The deadline miss and completion times are the two metrics to capture.
    \item Convert one task to interference task. An interference task can bump up its priority and/or overshoot the computation time. Show the impact on deadline misses and completion times.
    \item Put the 6 tasks in three containers. 2 task per container. Show deadline misses and completion times. This also should be configured to have no deadline misses even if the completion times suffer compared to first step.
    \item Repeat step 2 with containers. Let the interference task interfere within one of the containers only. Capture deadline misses and completion times. 2 containers should have no impact compared to step 3. One container, the one running interference, should show deadline misses and/or delayed completion times.
\end{enumerate}


\subsection{Real application}

Use a modularized car autopilot to demonstrate the application of the new scheduler. 

\begin{enumerate}
    \item Put each individual component of autopilot into separate containers. 
    \item Run the autopilot and make sure in this scenario everything works fine. 
    \item Run a interference task in core component, such as logging, to show that the core component are not affected. 
\end{enumerate}


% partitioned scheduler on multi-core, cite SCE paper, future work

% 1. Create an example with RR and TDMA pick some tasks and containers you have. Show in RR the task in safety critical container miss deadline and with TDMA that is not the case.

% 2. Performance does not get affected. 

% 3. Task in a certain criticality container are only affect by other tasks in that container. 

% 4. Show what context switch overhead between containers vs tasks within same container. 
%     1 higher priority task and 1 lower priority task. Hi task records timestamp before going to sleep. Then the low task records time when getting the CPU. 
%     Context switch overhead of processes from different containers and from same containers. 
    
% 5. Show how tasks in lower criticality containers get affected by tasks in high criticality containers
    








==> old file/5_related.tex <==
\section{Related Work}
\label{sec:relwork}

Safety critical applications need to have predictable execution and consistent availability. Limiting the impact of faults helps maximize the reliability and availability of the application. Creating isolation domains limits the potential impact of faults before they have been detected and provide granular entities for recovery by methods such as restarting these domains~\cite{abdi2018guaranteed}.
Various solutions have been proposed to use virtualized environments to run real time applications. The solutions belong to three broad categories.

\subsection{Single OS}
% Real Time OS~\cite{aroca2009real} are commercially available or open source OS that have features that reduce jitter in execution time and provide better control to applications on how resources are shared. For example, Linux's real time support reduces critical sections in the kernel to reduce jitter in preemption time and provides schedulers that implement real time scheduling algorithms, for example, SCHED\_DEALINE~\cite{lelli2016deadline}.
% Other solutions convert multi-core systems to a set of virtual single core systems~\cite{sce}. This is achieved by a strong isolation between any shared resources. But the strong guarantees come with the disadvantage of limiting communication between applications running on these virtual cores.
Single Core Equivalence (SCE)~\cite{sce} uses OS level techniques to create a set of virtual single-core platforms with strong performance isolation. SCE's primary focus is performance isolation to create virtual single core platforms. These isolation domains are intrinsically tied to the hardware. While some incidental data and fault isolation is provided by SCE, unlike containers, it does not offer the flexibility in scope of isolation domains or any protection to the shared OS from applications. The strong resource isolation guarantees also come with the disadvantage of limiting communication between applications running on these virtually isolated domains. It is still possible to combine the benefits of RT Containers proposed in this work with SCE. SCE creates virtual single core platforms from a multi-core platform. On each virtual core, RT containers can be used for single core scheduling and fault isolation among tasks running on this virtual core.

\subsection{Hypervisors}
Hypervisors allow multiple OS to share a hardware platform. The guest OSes run on virtually isolated hardware but only the hypervisor itself is aware of the sharing. Xtratum~\cite{masmano2009xtratum} and RT-Xen~\cite{xi2011rt} are hypervisors developed specifically for real-time and embedded systems. \cite{garcia2014challenges} lays out some of the challenges in running real time applications within hypervisors. Hypervisors provide strong isolation between guest applications, even if the application faults can impact the underlying OS. But this comes with high overheads that make this approach unsuitable for real time applications, specially when they run on resource constrained embedded platforms. 

\subsection{Containers}

Docker Containers provide process, filesystem, device, IPC, network and resource isolation between configurable domains called containers~\cite{bui2015analysis}. High overhead on hypervisor systems have steadily made containers, which have far lower overheads~\cite{soltesz2007container,seo2014performance}, the preferred technology for virtual isolation between applications running on shared hardware and OS.
Initial works explored the notion of containers as a distinctly schedulable entity and their scheduling with existing linux schedulers~\cite{wu2018dynamic,abeni2016container}.
RT-CASEs~\cite{cinque2019rt} extends real time containers to provide schdulability and fault isolation. In RT-CASEs tasks that exceed their worst case bounds only impact other tasks in the same container. Such faults do not impact tasks running in other containers independent of their relative criticality. It also features dynamic container management and monitoring.

Our work focuses on safety critical applications that run on resource constrained embedded systems. The application tasks have strict relative criticalities and priorities. Such a system favors lightweight solutions for hierarchical scheduling and fault isolation. Hence in this work we use containers as a lightweight fault and schedule isolation entity as required by the IMA standard. Any application level faults are fully limited to only tasks in the same container as the faulty tasks. This includes execution beyond expected worst case execution time and faulty changes in task priority at runtime. 

\cite{lee2000scheduling}
Scheduling tool and algorithm for integrated modular avionics systems
% \todo[inline]{List and summary start. This temporary list will be removed when we near final reviews.}


% \cite{lelli2016deadline}
% Deadline scheduling in the Linux kernel\\



% \subsection{Type 1}

% \cite{masmano2009xtratum} Xtratum: a hypervisor for safety critical embedded systems \\
% Type 1 hypervisor designed for RTS. Requires application modification to run bare. Hypervisor layer is non-preemptive.

% \cite{xi2011rt} RT-Xen: Towards real-time hypervisor scheduling in Xen \\
% Type 1 hypervisor which an RT modification for Xen.
% Extensive experimental results demonstrate the fea-
% sibility, eciency, and ecacy of xed-priority hierarchical
% real-time scheduling in RT-Xen. RT-Xen instantiates a suite
% of xed-priority servers (Deferrable Server, Periodic Server,
% Polling Server, and Sporadic Server).

% \cite{fautrel2019hypervisor} An hypervisor approach  for  mixed  critical  real-time  uav  applications\\
% Focused on schedulability analysis. 
% "Our first contribution is to provide conditions to decide on the schedulability of the tasks in their dedicated VM. 
% Second, we provide an algorithmic approach to compute slot durations."
% Schedule the most critical VM, the rest are harmonic period multiples. 
% Two level scheduling. Applications are scheduled by fixed priority inside VM.
% Used drone application as example for analysis.



% \subsection{Container Based}




% \cite{wu2018dynamic} Dynamic cpu allocation for docker containerized mixed-criticality real-time systems \\
% A scheduling for mixed RT and NRT containers setup. 
% Designed a new scheduler for Docker: Flexible Deferrable Server (FDS).
% Used CFS for RT container, focused on non-RT containers.
% For the RT aspect, it is guaranteed a container can use CPU up to quota us per period us.
% Flexible deferrable server (FDS) dynamically adjust cpu allocation for non-RT containers. Implemented in Docker community edition 17.09.0.


% \cite{melcher2018design} Design and implementation of a container-based architecture for real-time control applications \\
% This work proposed an architecture on using co-kernel to run real-time containers. 
% It focused more on the communication between containers.


% \cite{cinque2019rt}
% RT-CASEs: Container-Based Virtualization for Temporally Separated Mixed-Criticality Task Sets\\
% This is the main competing paper and requires an in-depth comparison in related work and implementation/evaluation.


% \cite{abeni2016container} Container-based  real-time scheduling  in  the  linux  kernel\\
% Container based realtime scheduling using native preempt Rt schedulers. 
% Almost identical to our scheduling part at least. 
% This paper extends the SCHED\_DEADLINE scheduling policy to a 2 level scheduling to schedule Linux control groups. 
% The control group is scheduled by SCHED\_DEADLINE and the user threads inside are to be scheduled with fixed priorities.

% \cite{cucinotta2019reducing}
% Reducing temporal interference in private clouds through real-time containers\\
% new hierarchical
% scheduling features of the SCHED\_DEADLINE real-time
% scheduler are exploited at the OS kernel level, in order to
% apply the resource reservation paradigm to isolate whole
% containers.


% \cite{de2019isolating}
% Isolating Real-Time Safety-Critical Embedded Systems via SGX-based Lightweight Virtualization\\
% In this position paper, we have discussed the adoption of
% both the Intel SGX hardware extension and the unikernel
% lightweight virtualization in the context of safety-critical realtime
% embedded systems.



% \todo[inline]{List and Summary end}


% \todo[inline]{Refine differences of our approach to existing as paper takes form.}

==> old file/6_conclusion.tex <==


\section{Conclusion}
\label{sec:conclusion}

==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{expl3, l3keys2e, xparse}
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
          \string\savepicturepage%
          {\pgfpictureid}{\noexpand\arabic{page}}%
        }%
      }%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
      \string\savepointas%
      {\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  if tikzmark on current page/.code n args={3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{%
      \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
        \pgfkeysalso{#3}%
      }{%
        \ifnum\csname save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname\endcsname=\the\value{page}\relax%
        \pgfkeysalso{#2}%
        \else
        \pgfkeysalso{#3}%
        \fi
      }%
    }%
  },
  if tikzmark on page/.code n args={4}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#4}%
    }{%
      \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}@label\endcsname}{%
        \pgfkeysalso{#4}%
      }{%
        \ifnum\csname save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname\endcsname=#2\relax%
        \pgfkeysalso{#3}%
        \else
        \pgfkeysalso{#4}%
        \fi
      }%
    }%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{%
  \csname pgfk@/tikz/tikzmark prefix\endcsname%
  #1%
  \csname pgfk@/tikz/tikzmark suffix\endcsname%
}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname%
  {\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tikzmarkalias#1#2{%
  \pgf@node@gnamelet{save@pt@#1}{save@pt@#2}%
  \pgf@node@gnamelet{save@pt@#1@offset}{save@pt@#2@offset}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
    \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}%
    \save@orig@pic%
    \pgfsys@getposition{\pgfpictureid}\save@this@pic%
    \pgf@process{\pgfpointorigin\save@this@pic}%
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\save@orig@pic}%
    \advance\pgf@x by -\pgf@xa
    \advance\pgf@y by -\pgf@ya
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process%
    {\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
        \edef\tmk@pg{\the\numexpr \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname - \csname save@pg@\pgfpictureid\endcsname\relax}%
        \ifnum \tmk@pg > 0 \relax
        \advance \pgf@xa by \pgf@x\relax
        \advance \pgf@ya by \pgf@y\relax
        \fi
        \ifnum \tmk@pg < 0 \relax
        \advance \pgf@xa by -\pgf@x\relax
        \advance \pgf@ya by -\pgf@y\relax
        \fi
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
  }%
}
\newcommand\tikzmark@outside[2][]{%
\tikz[remember picture with id=#2]{#1}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x}{\the\pgf@y}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \relax
  \ifx\scope\tikz@origscope\relax
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\arabic{page}}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark@outside}[2][]{%
    \only#3{\beameroriginal{\tikzmark@outside}[{#1}]{#2}}%
  }
  \renewcommand<>{\tikzmark@inside}[2]{%
    \only#3{\beameroriginal{\tikzmark@inside}{#1}{#2}}%
  }
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newif\iftikzmark@
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      #3%
    }{%
      #2%
    }%
}%
\newcommand\iftikzmarkexists[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false%
  }{%
    \tikzmark@true%
  }%
  \iftikzmark@
}%
\newcommand\iftikzmarkonpage[2]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname\endcsname=#2\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\newcommand\iftikzmarkoncurrentpage[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname\endcsname=\the\value{page}\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\def\subnode@#1#2#3{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  {%
    \let\pgf@sh@savedmacros=\pgfutil@empty% MW
    \let\pgf@sh@savedpoints=\pgfutil@empty%
    \def\pgf@sm@shape@name{rectangle}% CJ % TT added prefix!
    \pgf@sh@s@rectangle%
    \pgf@sh@savedpoints%
    \pgf@sh@savedmacros% MW
    \pgftransformshift{%
      \pgf@sh@reanchor{rectangle}{center}%
      \pgf@x=-\pgf@x%
      \pgf@y=-\pgf@y%
    }%
    \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
      \pgf@sh@reanchor{rectangle}{center}% FIXME : this is double work!
    }%
    % Save the saved points and the transformation matrix
    \edef\pgf@node@name{\tikz@fig@name}%
    \ifx\pgf@node@name\pgfutil@empty%
    \else%
    \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{rectangle}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
    \expandafter\pgf@sh@@temp\expandafter{%
      \pgf@sh@savedpoints}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
    \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
    \pgfgettransform\pgf@temp
    \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
    \fi%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}

\newcommand\subnode[3][]{%
  \ifmmode
  \mathchoice{%
    \subnode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \subnode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \subnode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \subnode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@#2}{%
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  }{}%
  \else
    \pgfnodealias{#2}{#2-d}%
    \tikzmarkalias{#2}{#2-d}%
  \fi
  \else
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  \fi
  \else
    \pgfnodealias{#2}{#2-s}%
    \tikzmarkalias{#2}{#2-s}%
  \fi
  \else
    \pgfnodealias{#2}{#2-ss}%
    \tikzmarkalias{#2}{#2-ss}%
  \fi
  \else
    \subnode@{#1}{#2}{#3}%
  \fi
}

\def\tikzmarknode@#1#2#3{%
  \tikz[%
    remember picture,
    baseline=(#2.base),
    save picture id={#2},
    every tikzmarknode picture/.try
  ] {
    \node[
      anchor=base,
      inner sep=0pt,
      minimum width=0pt,
      name={#2},
      node contents={#3},
      every tikzmarknode/.try,
      #1
  ]}%
}

\newcommand\tikzmarknode[3][]{%
  \ifmmode
  \mathchoice{%
    \tikzmarknode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@#2}{%
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  }{}%
  \else
    \pgfnodealias{#2}{#2-d}%
    \tikzmarkalias{#2}{#2-d}%
  \fi
  \else
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  \fi
  \else
    \pgfnodealias{#2}{#2-s}%
    \tikzmarkalias{#2}{#2-s}%
  \fi
  \else
    \pgfnodealias{#2}{#2-ss}%
    \tikzmarkalias{#2}{#2-ss}%
  \fi
  \else
    \tikzmarknode@{#1}{#2}{#3}%
  \fi
}
\def\usetikzmarklibrary{%
  \pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}%
  }%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let%
      \csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

\ExplSyntaxOn
\prop_new:N \g__sn_prop
\tl_new:N \l__sn_tmpa_tl
\tl_new:N \l__sn_tmpb_tl
\tl_new:N \l__open_bracket_tl
\tl_set:Nn  \l__open_bracket_tl {[} %]
\tl_new:N \l__sn_group_tl
\clist_new:N \l__sn_nodes_clist
\bool_new:N \l__sn_file_bool
\bool_new:N \g__sn_preamble_bool
\bool_set_true:N \g__sn_preamble_bool
\msg_new:nnn {tikzmark} {no file} {File~ "#1"~ doesn't~ exist.}
\msg_new:nnn {tikzmark} {loading nodes} {Loading~ nodes~ from~ "#1".}
\dim_new:N \l__sn_x_dim
\dim_new:N \l__sn_y_dim
\dim_new:N \l__sn_xa_dim
\dim_new:N \l__sn_ya_dim
\tl_new:N \l__sn_centre_tl

\tl_new:N \l__sn_transformation_tl
\tl_set:Nn \l__sn_transformation_tl {{1}{0}{0}{1}{0pt}{0pt}}
\iow_new:N \g__sn_stream
\bool_new:N \g__sn_stream_bool
\tl_new:N \g__sn_filename_tl
\tl_gset:Nx \g__sn_filename_tl {\c_sys_jobname_str}

\cs_new_nopar:Npn \sn_open_stream:
{
  \bool_if:NF \g__sn_stream_bool
  {
    \iow_open:Nn \g__sn_stream {\tl_use:N \g__sn_filename_tl .nodes}
    \bool_gset_true:N \g__sn_stream_bool
  }
}

\AtEndDocument
{
  \ExplSyntaxOn
  \bool_if:NT \g__sn_stream_bool
  {
    \iow_close:N \g__sn_stream
  }
  \ExplSyntaxOff
}
\makeatletter
\cs_set_eq:NN \tikz_set_node_name:n \tikz@pp@name
\cs_set_eq:NN \tikz_fig_must_be_named: \tikz@fig@mustbenamed

\cs_new_nopar:Npn \tikz_scan_point:n #1
{
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
}

\cs_new_nopar:Npn \tikz_scan_point:NNn #1#2#3
{
  \tikz@scan@one@point\pgfutil@firstofone#3\relax
  \dim_set_eq:NN #1 \pgf@x
  \dim_set_eq:NN #2 \pgf@y
}

\makeatother
\cs_generate_variant:Nn \tikz_scan_point:n {V}
\cs_generate_variant:Nn \tikz_scan_point:NNn {NNV}
\cs_new_nopar:Npn \save_nodes:Nn #1#2
{
  \tl_clear:N \l__sn_tmpa_tl
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(current~ bounding~ box.center)}
  \dim_set:Nn \l__sn_x_dim {-\l__sn_x_dim}
  \dim_set:Nn \l__sn_y_dim {-\l__sn_y_dim}
  \tl_set:Nx \l__sn_centre_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  }
  \clist_map_inline:nn {#2}
  {
    \tl_if_exist:cT {pgf@sh@ns@##1}
    {
      \clist_map_inline:nn {ns,np,ma,pi}
      {
        \tl_put_right:Nn \l__sn_tmpa_tl
        {
          \tl_gset:cn {pgf@sh@####1@ \tikz_set_node_name:n{##1} }
        }
        \tl_if_exist:cTF {pgf@sh@####1@##1}
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {
            {\exp_not:v {pgf@sh@####1@ \tikz_set_node_name:n {##1}}}
          }
        }
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {{}}
        }
      }
      \tl_put_right:Nn \l__sn_tmpa_tl
      {
        \tl_gset:cn {pgf@sh@nt@ \tikz_set_node_name:n{##1} }
      }
      \compose_transformations:NVv \l__sn_tmpb_tl \l__sn_centre_tl {pgf@sh@nt@##1}
      \tl_put_right:Nx \l__sn_tmpa_tl {{\exp_not:V \l__sn_tmpb_tl}}
      \tl_put_right:Nn \l__sn_tmpa_tl {
        \transform_node:Nn \l__sn_transformation_tl {
          \tikz_set_node_name:n{##1}
        }
      }
    }
  }
  \tl_set_eq:NN #1 \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_list:nn #1#2
{
  \save_nodes:Nn \l__sn_tmpa_tl {#2}
  \prop_gput:NnV \g__sn_prop {#1} \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_file:n #1
{
  \save_nodes:Nn \l__sn_tmpa_tl {#1}
  \sn_open_stream:
  \iow_now:Nx \g__sn_stream
  {
    \iow_newline:
    \exp_not:V \l__sn_tmpa_tl
    \iow_newline:
  }
}
\cs_generate_variant:Nn \save_nodes_to_list:nn {VV}
\cs_generate_variant:Nn \save_nodes_to_file:n {V}
\cs_new_nopar:Npn \restore_nodes_from_list:n #1
{
  \prop_get:NnNT \g__sn_prop {#1} \l__sn_tmpa_tl
  {
    \tl_use:N \l__sn_tmpa_tl
  }
}
\cs_new_nopar:Npn \restore_nodes_from_file:n #1
{
  \file_if_exist:nTF {#1.nodes}
  {
    \msg_log:nnn {tikzmark} {loading nodes} {#1}
    \ExplSyntaxOn
    \file_input:n {#1.nodes}
    \ExplSyntaxOff
  }
  {
    \msg_warning:nnn {tikzmark} {no file} {#1}
  }
}
\AtBeginDocument{\bool_gset_false:N \g__sn_preamble_bool}

\cs_new_nopar:Npn \compose_transformations:Nnn #1#2#3
{
  \tl_gset:Nx #1
  {
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {5}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {6}
      }
    }
  }
}
\cs_generate_variant:Nn \compose_transformations:Nnn {cVv,NVv,NVn,NvV,NnV}
\cs_new_nopar:Npn \transform_node:Nn #1#2
{
  \compose_transformations:cVv {pgf@sh@nt@#2} #1 {pgf@sh@nt@#2}
}
\cs_new_nopar:Npn \set_transform_from_node:n #1
{
  \tl_set_eq:Nc \l__sn_transformation_tl {pgf@sh@nt@#1}
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(#1.center)}

  \dim_set:Nn \l__sn_x_dim {\l__sn_x_dim - \tl_item:cn {pgf@sh@nt@#1}{5}}
  \dim_set:Nn \l__sn_y_dim {\l__sn_y_dim - \tl_item:cn {pgf@sh@nt@#1}{6}}

  \compose_transformations:NnV  \l__sn_transformation_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  } \l__sn_transformation_tl
}
\cs_generate_variant:Nn \set_transform_from_node:n {v}
\tikzset{
  set~ saved~ nodes~ file~ name/.code={
    \tl_gset:Nx \g__sn_filename_tl {#1}
  },
  transform~ saved~ nodes/.code={
    \set_transform_from_node:v {tikz@last@fig@name}
  },
  set~ node~ group/.code={
    \tl_set:Nn \l__sn_group_tl {#1}
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ nodes~ to~ file/.code={
    \tl_if_eq:nnTF {#1}{false}
    {
      \bool_set_false:N \l__sn_file_bool
    }
    {
      \bool_set_true:N \l__sn_file_bool
    }
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ node/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \clist_gput_right:Nv \l__sn_nodes_clist {tikz@last@fig@name}
        }
      }
    }
  },
  restore~ nodes~ from~ file/.code={
    \bool_if:NTF \g__sn_preamble_bool
    {
      \restore_nodes_from_file:n {#1}
    }
    {
      \tikz_fig_must_be_named:
      \pgfkeysalso{append~ after~ command={
          \pgfextra{
            \scope
            \split_argument:NNn \tikzset \restore_nodes_from_file:n {#1}
            \endscope
          }
        }
      }
    }
  },
  restore~ nodes~ from~ file/.default = \g__sn_filename_tl,
  restore~ nodes~ from~ list/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \scope
          \split_argument:NNn \tikzset \restore_nodes_from_list:n {#1}
          \endscope
        }
      }
    }
  }
}
\cs_generate_variant:Nn \clist_gput_right:Nn {Nv}
\cs_new_nopar:Npn \split_argument:NNn #1#2#3
{
  \tl_set:Nx \l__sn_tmpa_tl {\tl_head:n {#3}}
  \tl_if_eq:NNTF \l__sn_tmpa_tl \l__open_bracket_tl
  {
    \split_argument_aux:NNp #1#2#3
  }
  {
    #2 {#3}
  }
}
\cs_new_nopar:Npn \split_argument_aux:NNp #1#2[#3]#4
{
  #1 {#3}
  #2 {#4}
}
\cs_new_nopar:Npn \maybe_save_nodes:
{
  \clist_if_empty:NF \l__sn_nodes_clist
  {
    \bool_if:NTF \l__sn_file_bool
    {
      \save_nodes_to_file:V \l__sn_nodes_clist
    }
    {
      \tl_if_empty:NF \l__sn_group_tl
      {
        \save_nodes_to_list:VV \l__sn_group_tl \l__sn_nodes_clist
      }
    }
    \clist_gclear:N \l__sn_nodes_clist
  }
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2011-2018 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> tikzmarklibrarylistings.code.tex <==
%%
%% This is file `tikzmarklibrarylistings.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `listings')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\@ifpackageloaded{listings}{%
    \newif\iflst@linemark
\lst@AddToHook{EveryLine}{%
  \begingroup
  \advance\c@lstnumber by 1\relax
  \pgfmark{line-\lst@name-\the\c@lstnumber-start}%
  \endgroup
}
\lst@AddToHook{EOL}{\pgfmark{line-\lst@name-\the\c@lstnumber-end}%
\global\lst@linemarktrue
}
\lst@AddToHook{OutputBox}{%
  \iflst@linemark
  \pgfmark{line-\lst@name-\the\c@lstnumber-first}%
  \global\lst@linemarkfalse
  \fi
}
\def\tkzmk@lst@fnum#1\relax#2\@STOP{%
  \def\@test{#2}%
  \ifx\@test\@empty
  \def\tkzmk@lst@start{0}%
  \else
  \@tempcnta=#1\relax
  \advance\@tempcnta by -1\relax
  \def\tkzmk@lst@start{\the\@tempcnta}%
  \fi
}
\lst@AddToHook{Init}{%
  \expandafter\tkzmk@lst@fnum\lst@firstnumber\relax\@STOP
  \pgfmark{line-\lst@name-\tkzmk@lst@start-start}%
}
}{%
    \PackageError{tikzmark listings}{The listings package has not been loaded.}{}
}
%% 
%% Copyright (C) 2011-2018 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzmarklibrarylistings.code.tex'.

